Towards Automated Solution Recipe Generation for Industrial Asset Management with LLM

This study introduces a novel approach to Industrial Asset Management (IAM) by incorporating Conditional-Based Management (CBM) principles with the latest advancements in Large Language Models (LLMs). Our research introduces an automated model-building process, traditionally reliant on intensive collaboration between data scientists and domain experts. We present two primary innovations: a taxonomy-guided prompting generation that facilitates the automatic creation of AI solution recipes and a set of LLM pipelines designed to produce a solution recipe containing a set of artifacts composed of documents, sample data, and models for IAM. These pipelines, guided by standardized principles, enable the generation of initial solution templates for heterogeneous asset classes without direct human input, reducing reliance on extensive domain knowledge and enhancing automation. We evaluate our methodology by assessing asset health and sustainability across a spectrum of ten asset classes. Our findings illustrate the potential of LLMs and taxonomy-based LLM prompting pipelines in transforming asset management, offering a blueprint for subsequent research and development initiatives to be integrated into a rapid client solution.

==> sections/SelfAlignQuestions.tex <==
\section{Solution Outline}
\vspace{10pt}




==> sections/discussion.tex <==
\section{Discussion}
\vspace{10pt}

This paper highlights the significant role Large Language Models (LLMs) play in enhancing condition-based maintenance strategies within industrial settings. Our experimental results demonstrate that, when equipped with an adaptable prompt template enriched by industry-specific domain data, LLMs emerge as a formidable tool in bolstering maintenance decision-making processes. Specifically, these models excel in pinpointing key performance indicators (KPIs) that are pivotal for informing targeted maintenance activities, taking into account the nuances of data availability. This plays a crucial role in practical settings when stakeholders are faced with industrial assets containing multiple components and a wide variety of IoT sensors. The continuing specialization of industrial assets is adding to this heterogeneity of both metadata defining the asset and IoT data defining the condition of the asset

Our results indicate that infusing domain-specific data within prompts and effectively sequencing prompts is critical to enhancing the value of LLMs to typical CBM tasks. The provision of comprehensive details concerning each asset, including its unique operational challenges, is indispensable for customizing the deployment of LLMs. Such customization is vital for harnessing the full potential of these models, thereby ensuring that the maintenance activities are not only predictive but also optimally aligned with the specific needs and constraints of each asset.

This tailored approach, facilitated by LLMs, represents a leap forward in maintenance practices. By enabling a more nuanced and data-informed maintenance strategy, LLMs contribute to the reduction of unnecessary downtime and maintenance costs, while simultaneously enhancing the longevity and reliability of critical industrial assets.







In the discussion, we want to provide a clear and concise overview of how the integration of these three critical factors can revolutionize industrial asset management. The table format offers a structured way to visualize the relationship and interdependencies among the meta-model, LLM, and asset-specific challenges.  


The convergence of a meta-model framework, the selection of appropriate Large Language Models (LLM), and the precise identification of asset types and their associated challenges represent a groundbreaking approach in industrial asset management. This "marriage" of key elements forms a robust and dynamic system capable of addressing complex industrial problems with unprecedented efficiency and accuracy.

    Meta-Model Framework: Serves as the foundational structure, encapsulating the overarching principles and variables relevant to various asset types and maintenance strategies.

    Large Language Models (LLM): Provide the computational power and advanced analytics capabilities, enabling deep insights and predictive accuracy that were previously unattainable.

    Asset Type and Problem Identification: The specific nature of each asset and its unique challenges are crucial for tailoring the meta-model and LLM application to achieve optimal results.

The following table illustrates the interplay of these factors, showcasing how they collectively contribute to a more intelligent and responsive asset management system:




==> sections/experiment_case_study_save.tex <==
\section{Experiment}
\vspace{10pt}

In this section, we delve into the experimental phase of our study, focusing on applying our methodology to the generation of asset health scores, a standard KPI required for asset management. This experiment aims to validate the efficacy of our approach and serve as a testament to the robustness and versatility of different asset classes. 

\subsection{Experiment}
\vspace{10pt}

Our experiments focused on evaluating two critical Key Performance Indicators (KPIs) for asset classes: the health and sustainability scores. The health score serves as a measure to assess the condition of an asset. We adopted two significant perspectives to estimate this score: monitoring individual components and analyzing historical maintenance and repair records. Its unique taxonomy and corresponding prompt design underpinned each view, allowing for nuanced and targeted assessments. Conversely, the sustainability score was examined as a vital KPI to gauge the asset's environmental impact, particularly its contributions to global warming. 

In the remaining discussion, we focus on The health score experiment is the focus of the  from IBM Maximo Asset Score~\footnote{\url{http://maximo-lab.monitordemo4.ibmmam.com/apm_8.9/asset_scores}}

The website discusses "Asset Custom Scores" in Maximo Health and Maximo Health and Predict - Utilities (HPU) within the Maximo Application Suite (MAS). It focuses on new features allowing users to create custom scores for asset conditions using either a formula-based approach or notebook-based methods deployed through Watson Studio or IBM Machine Learning Service. These custom scores help make informed repair or replacement decisions and select assets for investment projects. The page also highlights a lab exercise demonstrating how to set up and use these scores, prerequisites for the lab, and the use of Maximo Health for asset condition analysis and investment strategy optimization. The content is aimed at reliability engineers and subject matter experts in asset management.

\subsection{Knowledge Extraction}
\vspace{10pt}

In the experimental phase of our knowledge extraction, we meticulously tested four distinct approaches to generate outputs for the knowledge base, specifically tailored to the domain of a given Key Performance Indicator (KPI). Our initial step involved compiling a comprehensive list of questions. Among these, we identified a crucial element: the final question in our guided pipeline, which plays a pivotal role in the process.

The approaches tested are as follows:

    \begin{itemize}
        \item Single Question (SQ): This approach focuses on the last question in the guided pipeline, isolating its potential to elicit comprehensive information.
        
        \item All Questions Concatenated (AllQ): Here, we combined all questions into one extended query, testing the effect of presenting the full context in a single prompt.
         
        \item All Questions with Chain of Thought (AllQCOT): This method enhances the AllQ approach by incorporating a 'think step-by-step' comment in the prompt, guiding the LLM to process the information in a structured, sequential manner to follow a reasoning process by explicitly laying out the intermediate steps leading to the desired outcome. This approach goes beyond simply providing input and output but allows the model to "show its work" and demonstrate its understanding of the problem.
        
        \item Guided Iterative Process (GIP): This approach simulates a dynamic Q/A session, where each question and its subsequent answer lead to the next query, mirroring a real-world interaction pattern.  In this process, there are multiple Q/A generated and such answers help to understand how the final knowledge is generated for better validation with a human-in-the-loop. 
        \item 
    \end{itemize}
    
Each of these methods aims to optimize the extraction of domain-specific knowledge for a particular KPI, evaluating their effectiveness in contributing to a rich, accurate knowledge base. This experimentation is crucial in determining the most efficient approach to harnessing the capabilities of LLMs for detailed and relevant knowledge generation in industrial asset management.
        

\begin{table*}[h]
\centering
\caption{Summary of Methods and Their Advantages and Disadvantages}
\begin{tabular}{>{\raggedright\arraybackslash}p{3.5cm} >{\raggedright\arraybackslash}p{5.0cm} >{\raggedright\arraybackslash}p{5.5cm}}
\toprule
\textbf{Method} & \textbf{Advantages} & \textbf{Disadvantages} \\
\midrule
Single Question (SQ) & Focus and precision, Simplicity in execution & May miss broader context, Limited in scope \\
\addlinespace
All Questions Concatenated (AllQ) & Contextual richness, Holistic understanding & Potentially overwhelming for the model, May produce less focused responses \\
\addlinespace
All Questions with Chain of Thought (AllQCOT) & Structured thinking, Enhanced clarity & More complex to construct, May lead to verbose responses \\
\addlinespace
Guided Iterative Process (GIP) & Dynamic interaction, Incremental learning, Customizability & Time-consuming, Requires careful question crafting \\
\bottomrule
\end{tabular}
\end{table*}


\subsection{Knowledge to Code}
\vspace{10pt}

\subsubsection{Sample Data Generation}
\vspace{10pt}

We have two approaches to generate the sample data.  One is directly from the code, 

\subsubsection{Experiment Categories and Objectives}
\vspace{10pt}


\subsubsection{Experiment Components}
\vspace{10pt}

Each problem category involves three key components: 
\begin{itemize}
    \item \textbf{Documentation:} Structure and format of Markdown files for documentation.
    \item \textbf{Configuration:} Model configurations and parameter adjustments.
    \item \textbf{Python Code:} Python code structure, compatibility with MLFlow and Model Factory.
\end{itemize}


\subsection{Case Study - Health Score for Industrial Assets}
\vspace{10pt}


Using the health score as an example,  we separate the health score analyzed from three aspects:
1. the component qualities; 
2. the historical records;
3. the asset ages.

We develop the health score for each of the aspects independently.  The end-user has the freedom to select and choice which aspects based on the data availability. 


\subsection{Validation}
\vspace{10pt}

There are multiple validations required for the recipe for the artifacts.  Certain artifacts are likely to be validates, within all the artifacts, the most important one is the knowledge documents.

As illustrated in Figure~\ref{fig:Pipelines for Artifact Generation}, the initial artifacts comprise a knowledge document outlining methods for estimating or modeling a Key Performance Indicator (KPI). Subsequent recipe artifacts are then deduced from this foundational knowledge. However, a critical aspect of our research involves validating these artifacts to ensure their utility and reliability.  It is imperative to validate knowledge document validation.

Validation hinges on two key factors: completeness and accuracy. While our current research predominantly focuses on reducing hallucinations in the generated content, our standards go beyond this. It is imperative that the generated document not only adheres to a specific format but also encompasses accurate, relevant, and comprehensive information.

Yet, assessing completeness presents a significant challenge, as it is inherently difficult to quantify. A conventional approach would involve creating a similar document manually and performing a similarity comparison. However, in our case, such pre-existing documents do not exist; this creates a 'chicken and egg' problem. Without prior knowledge or a benchmark document, evaluating the completeness of our generated artifacts becomes a complex task that may require innovative validation methodologies tailored to the unique nature of our project.


==> sections/introduction_save.tex <==
\section{Introduction}
\vspace{10pt}


LLM and moving to a specific area. 
Asset Management Development towards the CBD
Challenging applying to Asset Management
Contribution from us
Paper Organization

In the rapidly evolving landscape of industrial advancement, the integration of asset-specific management with cutting-edge technological innovations, particularly Large Language Models (LLM), has become increasingly vital. This integration, however, presents distinct challenges, primarily in aligning domain-specific expertise with the advanced capabilities of data science. A significant gap exists in the ability of any individual to effectively bridge these complex domains. Traditionally, this bridging has involved collaborative efforts among industrial domain experts, such as site engineers, data scientists skilled in sophisticated modeling, and software engineers tasked with converting these insights into reusable components. This process, often reliant on extensive Q/A sessions and brainstorming, tends to be time-consuming, challenging, and costly.

The introduction of LLM into this dynamic changes the paradigm significantly. LLMs have the potential to drastically reduce the effort required from each stakeholder, streamlining the process of integrating domain knowledge with data science and software engineering. By automating aspects of knowledge extraction, model development, and code generation, LLMs can facilitate a more efficient and seamless collaboration between domain experts, data scientists, and software engineers. This paper aims to explore these opportunities, focusing on how LLM can alleviate the critical pain points in the development process within the realm of industrial solutions. Through this exploration, we seek to demonstrate how LLM can not only expedite the development process but also enhance the accuracy and applicability of industrial management strategies, leading to more effective and cost-efficient solutions.



To address these complexities, we introduce the concept of the Large Language Model (LLM). Our approach is grounded in the synergy of domain-specific knowledge and advanced data science techniques. The LLM framework we propose leverages the foundational principles of management while integrating insights from diverse resources, including technical forums like Stack Overflow. This integration enables the LLM to exhibit a profound understanding of both domain-specific requirements and data science methodologies, thus bridging the existing gap in the field.

Generalist foundation models such as GPT-4 from OpenAI, Llama-2 from Meta have displayed surprising capabilities in a wide variety of domains and tasks. Yet, there is a prevalent assumption that they cannot match specialist capabilities without intensive training of models with specialty knowledge.  We build on a prior study of the specialist capabilities of LLM on medical challenge benchmarks in the absence of special training. In distinction to the intentional use of simple prompting to highlight the model’s outof-the-box capabilities, we perform a systematic exploration of prompt engineering to boost performance. We find that prompting innovation can unlock deeper specialist capabilities and show that GPT-4 easily tops prior leading results for medical question-answering datasets. The prompt engineering methods we explore are general purpose, and make no specific use of domain expertise, removing the need for expert-curated content. Our experimental design carefully controls for overfitting during the prompt engineering process. As a culmination of the study, we introduce Medprompt, based on a composition of several prompting strategies. Medprompt greatly enhances GPT-4’s performance and achieves state of the art results on all nine of the benchmark datasets in the MultiMedQA suite. The method outperforms state-ofthe-art specialist models such as Med-PaLM 2 by a large margin with an order of magnitude fewer calls to the model. Steering GPT-4 with Medprompt achieves a 27\% reduction in error rate on the MedQA dataset (USMLE exam) over the best methods to date achieved with specialist models, and surpasses a score of 90\% for the first time. Moving beyond medical challenge problems, we show the power of Medprompt to generalize to other domains and provide evidence for the broad applicability of the approach via studies of the strategy on competency exams in electrical engineering, machine learning, philosophy, accounting, law, nursing, and clinical psychology.


The practical application of our approach is demonstrated through a case study involving the Llama-2-chat model, applied in the context of managing electrical transformers. Firstly, This case study serves as a template for the formulation of our solution. Secondly, it is a testament to the model's capability to comprehend and address complex domain-specific challenges. It highlights the model's adaptability and its proficiency in generating effective solutions tailored to the unique demands of industrial management.


\subsection{Outline of Possible Solution}
\vspace{10pt}

\subsection{Contribution}
\vspace{10pt}

This paper makes pivotal contributions to the integration of Large Language Models (LLM) in industrial asset management, setting a new standard in the fusion of domain expertise and data science:

    Practical Application of LLM: We demonstrate the practical application of LLM in industrial settings, bridging the gap between domain knowledge and data science. This approach enhances the adaptability and efficiency of solutions, providing valuable insights for future AI applications in industrial management.

    Guided Auto-Recipe System for Efficient Management: From a business perspective, our guided auto-recipe system revolutionizes industrial asset management. This innovative system significantly reduces the time and resources required for model development, offering a seamless methodology for managing diverse assets and improving reliability and efficiency, particularly in wind turbine gearboxes.

    Technical Advancements in LLM Application: Technically, we advance the application of LLM through:
        Knowledge Acquisition and Implementation: Employing a guided approach with LLM for streamlined documentation, configuration, and coding.
        Cross-Domain Transfer Learning: Demonstrating LLM's capability for transfer learning across various industrial domains, enhancing the integration and efficiency of asset management practices.
        Cognitive Meta-Model for Guidance: Introducing a cognitive meta-model to guide the integration of LLM in industrial processes, ensuring tailored and effective solutions.

These contributions collectively mark a significant leap in the use of LLM for industrial asset management, offering a comprehensive framework for its application and underscoring the potential for enhanced efficiency and effectiveness in the field.

\subsection{Remaining Paper  Organization}
\vspace{10pt}

The paper is organized as follows.  Section II introduces the problem formulation that focuses on the background of conditional asset management and standardization of the KPIs and modeling practices to ensure an easy knowledge extraction from LLM.  Section III outlines the solution.  We mainly focus on how to extract domain-specific knowledge for selected asset types automatically.  Section IV provides the results from different LLM models to demonstrate the feasibility of this approach and the code base for such automation.  Section V provides detailed examples of electrical transformers.  Section VI provides the summary and future perspective. 
The paper is organized as follows.  Section II introduces the problem formulation that focuses on the background of conditional asset management and standardization of the KPIs and modeling practices to ensure an easy knowledge extraction from LLM.  Section III outlines the solution.  We mainly focus on how to extract domain-specific knowledge for selected asset types automatically.  Section IV provides the results from different LLM models to demonstrate the feasibility of this approach and the code base for such automation.  Section V provides detailed examples of electrical transformers.  Section VI provides the summary and future perspective. 

==> sections/introduction_save_020124.tex <==
\section{Introduction}
\vspace{10pt}

For decades, industrial asset management echoed the cadence of fixed schedules and standardized practices epitomized by frameworks like ISO 55001~\footnote{https://www.iso.org/standard/55089.html}. While once effective, these rigid approaches struggle to adapt to the evolving demands of modern environments. The emergence of data-rich ecosystems, pulsating with interconnected sensors and the industrial Internet of Things (IoT), necessitates a paradigm shift towards conditional asset management, a cornerstone of Industry 4.0 \citep{fernandes2021role}. This data-centric method moves away from set maintenance schedules towards a system refined by IoT insights. Merging key performance indicators (KPIs) regarding asset health, failure scenarios, operational efficiency, and past maintenance actions with sensor data and predictive analytics introduces a flexible maintenance framework. This framework easily adjusts to the various requirements of an efficient maintenance strategy. CBM ensures improved effectiveness, decreased downtime, and better allocation of limited resources like labor and components.
%It weaves a dynamic tapestry of equipment health and performance gleaned from the ever-vigilant gaze of IoT sensors. Advanced analytics become the conductor, orchestrating this symphony of data into prescient forecasts of potential failures. Maintenance transforms from a reactive waltz to a proactive ballet, performed only when the data sings its urgent aria. By embracing this dynamic perspective, organizations unlock a new era of efficiency, where downtime pirouettes away and resource utilization takes center stage, paving the way for a future where conditional asset management dances in perfect harmony with the aspirations of the intelligent factory.

\begin{comment}
While embracing this dynamic perspective in asset management offers numerous advantages, it also introduces complex challenges. While IoT and predictive analytics plays a key role, it’s crucial to recognize that CBM necessitates a comprehensive understanding of various factors, including asset health and associated costs. Although the general philosophy and methodology of condition-based management remain consistent across asset types, the processes for integrating IoT data and generating KPIs vary considerably. This variability underscores the need for in-depth domain knowledge and a nuanced understanding of individual assets and operational requirements of each organization. Translating IoT data into actionable insights for decision support presents a significant challenge for data scientists. Consequently, there is a pressing need for methods that expedite the acquisition of such specialized knowledge, thereby accelerating the development of tailored solutions for individual asset types. This aligns with the larger goal of enhancing the efficiency and effectiveness of asset management in the context of IoT and Industry 4.0.


\textcolor{red}{This paragraph is kind of repetitive of what's above. Think we can drop}
\end{comment}

%However, the practical implementation of Condition-Based Maintenance (CBM) presents significant challenges and is labor-intensive. A notable gap exists between the conceptual framework of CBM and its real-world application. The transition from conceptual KPIs, general cross-industrial application domains, to effective decision-support systems is complex. Key Performance Indicators such as performance efficiency, health, sustainability, and manageability scores become critical in this process. These indicators serve as foundational elements for decision support. Each asset type demands specific domain knowledge, further complicating the implementation process. Compounding this complexity is that individual assets or fleets often exhibit unique characteristics stemming from vendor differences, operational conditions, and the types of sensors deployed. Starting from scratch to tailor CBM for each client becomes costly, potentially leading to reluctance to adopt and adapt such solutions.  In summary, the challenges in implementing CBM arise primarily from two sources: the diversity of asset types and the diversity of client needs and contexts. Bridging these gaps is essential for successfully integrating CBM in industrial asset management. The question then becomes: how can we effectively bridge these gaps, creating a more universally adaptable yet customizable CBM framework?

The practical implementation of Condition-Based Maintenance (CBM) faces notable challenges, primarily due to the need for more automation in current solutions.  A substantial gap exists between the theoretical underpinnings of CBM and its operationalization, particularly in translating conceptual Key Performance Indicators (KPIs) and cross-industrial applications into effective decision-support systems with complexity and labor-intensive activities for data scientists.  The implementation challenge is further compounded by the need for specific domain knowledge for each asset type, alongside the unique characteristics of individual assets or fleets, which may vary due to differences in vendors, operational conditions, and sensor types used.  How can we develop a universally adaptable and customizable framework for different KPIs required for decision support?  The advent of large language models (LLMs) presents an opportunity to bridge this gap, marking our pioneering research in this specific problem domain.

In addressing the challenges of KPI modeling for specific asset types in Condition-Based Maintenance (CBM), the concept of a ``solution recipe" emerges as a core component. A solution recipe is a collection of artifacts, readily deployable within a standardized environment such as a model factory. These serve to actualize a CBM solution or, more broadly, facilitate context-aware, data-driven asset management. These artifacts encompass four primary categories: documents, configuration files, code, and sample data. Notably, programming code plays a critical role in converting IoT data into meaningful KPIs, ensuring that the method is both reliable and understandable. These models can be categorized as either engineering-based, which are established on recognized mechanistic or empirical relationships, or as those depending on machine learning algorithms. The latter includes techniques like anomaly detection, failure prediction, and assessment of the expected lifespan of assets.

The availability of domain-specific solution recipes can significantly expedite the CBM implementation process. However, the development and fine-tuning of such automated solutions necessitate extensive collaboration. This collaboration involves decision-makers, site engineers, domain experts, and data scientists working in unison. A key question in this context is the feasibility of streamlining and automating this collaborative step.
%Exploring this possibility forms the crux of our research, aiming to enhance the efficiency and adaptability of CBM in diverse industrial settings.

Currently, LLMs are gaining prominence across diverse sectors, showing remarkable capabilities from healthcare to finance. In healthcare, for example, LLMs aid in complex tasks such as analyzing medical records and creating tailored healthcare strategies. The integration of LLMs in industrial asset management is currently in its infancy, largely owing to the specialized nature of operational tasks and the essential need for a multidisciplinary approach in decision-making processes.

The advent of LLMs in asset management corresponds with the idea of employing solution recipes to create an organized depiction of maintenance information at the asset level. If the generation of these solution recipes can be automated for different KPIs, such recipes could form a foundational basis for bridging the gap between low-level sensor monitoring and predictive analytics towards high-level intelligent asset management. This integration signifies a pivotal transformation, where LLMs synthesize intricate sensor and asset data into strategic insights, propelling asset management into a new era of intelligence and efficiency.


Although direct user interaction with an LLM can inform CBM, its effectiveness is often restricted by the complexity inherent to asset maintenance. Instead, we propose a method combining specialized industry knowledge, uniform KPIs, and generated code recipes to boost performance. This provides a more systematic approach to organizing LLM output into a structured form suitable for diverse asset types. %Consequently, a simple free-text chat interface does not suffice; there is a need for a more comprehensive workflow to handle this complexity. A critical challenge lies in that LLMs can generate similar outputs across different asset types, undermining the specificity required for effective CBM.

%Building upon this transformative potential, this paper introduces a novel approach titled ``Unlocking the Power of Metadata: Meta-Taxonomies for Efficient Knowledge Extraction and Aggregation for Industrial Asset Management." \textcolor{red}{Is this the title of the paper or what exactly is it?} 
This approach aims to mimic the mental process of devising solutions for specific KPIs. The term 'meta-taxonomy' is employed to reflect the abstraction of this process; rather than focusing on asset-specific details, it creates placeholders for knowledge extraction, enhancing the adaptability of the framework. Implementing these meta-taxonomies is a crucial step in maximizing the efficacy of LLMs within industrial asset management. By facilitating the extraction and generation of actionable insights, these structured systems are tailored to meet different asset types' specific needs and nuances. This development underscores the versatility of LLMs in industrial applications. It marks a strategic advancement in industrial asset management, leveraging AI to achieve unprecedented customization and efficiency.

\subsection{Contribution}
\vspace{10pt}

Our research significantly advance the integration of Large Language Models (LLMs) in industrial asset management, across the following key areas:

\begin{itemize}
    \item \textbf{Practical Application of LLMs}: We bridge the theoretical potential and practical utility of LLMs in engineering applications. This exploration opens avenues for generative AI applications in varied industrial contexts, demonstrating the real-world benefits and practicality of LLM integration.
    \item \textbf{Guided Auto-Recipe System}: From a business standpoint, our system innovates in the management of industrial assets. It streamlines development processes, reducing time and resources required, while enhancing asset management and reliability. This approach represents an unparalleled methodology for handling diverse assets efficiently.
    \item \textbf{Technical Advancements in LLM Application}: Our work expands the capabilities of LLMs in several dimensions, including knowledge acquisition and implementation, cross-domain transfer learning, and cognitive meta-model for guidance.   We are using the guided (or constrained reasoning) with the help of meta-taxonomy to solve the KPI calculation or estimation problem. The solution is the output as a recipe containing a list of the artifacts to allow crafting to specific clients needs and data availability.
    \item \textbf{Standardization of Chain-of-Thought in CBM KPIs and Metrics}: We have standardized the chain-of-thought process using the meta-taxonomy for Condition-Based Maintenance (CBM) Key Performance Indicators (KPIs) and metrics, enhancing the clarity and consistency of decision-making processes in asset management.
\end{itemize}

Furthermore, our approach formulates industrial problems using a meta-taxonomy designed for generating AI-driven recipes through LLMs. This methodology marks a significant departure from existing deep learning models and plays a crucial role in Condition-Based Maintenance (CBM). A key innovation lies in the taxonomy's adaptability, which can be dynamically updated to accommodate new assets using LLMs—a feature not yet explored in current literature.

Addressing user accessibility, our research generates hierarchical taxonomy-based questions to assist end-users. The development of a comprehensive pipeline, incorporating various roles, is aimed at generating necessary artifacts for a complete AI recipe.

These contributions collectively herald a new era of efficiency and effectiveness in industrial asset management, highlighting the transformative potential of LLMs and meta-taxonomies.


\subsection{Remaining Paper  Organization}
\vspace{10pt}

The paper is organized as follows.  Section II introduces the problem formulation that focuses on the background of conditional asset management and standardization of the KPIs and modeling practices to ensure an easy knowledge extraction from LLM.  Section III outlines the solution.  We primarily focus on how to automate domain-specific knowledge extraction for selected asset types.  Section IV evaluates the results across multiple different LLMs and assesses the feasibility of the approach.  Section V considers case study focusing on electrical transformers.  Section VI provides the summary and future perspective. 
The paper is organized as follows.  Section II introduces the problem formulation that focuses on the background of conditional based maintenance and standardization of the KPIs and modeling practices to enhance asset management.  Section III outlines the solution.  We mainly focus on how to extract domain-specific knowledge for selected asset types automatically.  Section IV provides the results from different LLM models to demonstrate the feasibility of this approach and the code base for such automation.  Section V provides detailed examples of electrical transformers.  Section VI provides the summary and future perspective. 

==> sections/notes.tex <==

We have a DAG to define a workflow to outline the solution process.  We assume that the nature of the problem for different asset types is similar. However, the difference depends on the 

Same business problems, same 

Health Agent
    Give Me a Health Score, a function of another score with weight.  The weight is defined by the asset type (LLM).  How many scores are required? 

    A. Mechanical, B. Thermal, C. Electrical; D Chemical 
    
AnaAgent
Failure Agent

Multiple steps of the workflow: The agents should follow numerous workflows.

A->B->C->D

A->B->C->D 

Health Score for the Wind Turbine Gearbox

Output
1. Recipe, 2. document, 3. Configuration; 4. Python Code

Tools:

Model Factory: Receipt
Monitor:  Generate the necessary 

roles of Agents:

1.  Data Scientist Agent
2.  Domain Agent
3.  System Agent



==> sections/problem_formulation_new.tex <==
\section{Problem Formulation}
The problem we are addressing in our research is how to create a comprehensive solution using LLM that automatically generates a recipe for a specific industrial asset based on one Key Performance Indicator (KPI). 

% Conditional based maintenance in industrial asset management is data-centric and heavily dependent on domain knowledge. Traditional asset management methods are often labor-intensive and rigid, struggling to adapt to the unique demands of various asset classes and the complexities associated with different Key Performance Indicators (KPIs) (see Table~\ref{tab:list_kpis}) and key metrics using data-driven approach (see Figure~\ref{fig:industrical_solution}). 

% Our problem formulation centers on a dynamic data-driven automated solution that not only resolves the weakness of the traditional asset management methods but also leverages the potential of Large Language Models (LLMs) and Taxonomy-aware prompting. By tackling this problem, the goal is to revolutionize asset management by significantly enhancing efficiency, adaptability, and precision in maintenance and decision-making processes.

\subsection{Key Terms: KPIs, Metrics and Sensors}
Key Performance Indicators (KPIs) are the strategic measures closely linked to overarching business goals. Metrics are a broader range of operational measurements detailing various aspects of asset performance.  Both are essential for evaluating and enhancing asset performance, implementing maintenance strategies, and guiding investment decisions. The KPIs/metrics, such as mean-time-between-failure (MTBF), maintenance costs, and asset availability, provide tangible measures of an asset's operational efficiency and performance. Meanwhile, The KPIs/metrics, like failure probability, component condition monitoring, and greenhouse gas equivalent emissions, offer predictive insights, enabling the assessment of asset risk, asset health, and their environmental impact. These indicators guide informed decisions about maintenance practices, resource distribution, and long-term asset strategy formulation. Table ~\ref{tab:KPIs} lists eight KPIs commonly used in industrial asset management sectors.%\textcolor{red}{A reference for this would make it more convicing. Is there a maximo manual or something we can cite. Do we need a KPI for asset running cost or is performance efficiency a proxy}.

\begin{table}[!h]
\centering
\small
\caption{KPIs for Industrial Asset}
\begin{tabular}{>{\raggedright\arraybackslash}p{2.5cm} >{\raggedright\arraybackslash}p{5.0cm} >{\raggedright\arraybackslash}p{2.5cm}}
\toprule
\textbf{KPIs} & \textbf{Meaning} \\
\midrule
Health Score & Reflects the current condition and performance of an asset. \\ \hline
Sustainability Score & Evaluates the environmental sustainability of asset operations \\ \hline
Asset Reliability & Measures the frequency of asset functioning without failure \\ \hline
Maintenance Costs & Tracks the costs associated with maintaining an asset \\ \hline
Asset Availability & Proportion of time an asset is operational and available for use. \\ \hline
Performance Efficiency & Assesses the operational effectiveness of an asset. \\ \hline
Reliability Score & Indicates the dependability of an asset over time \\ \hline
Criticality Score & Assesses the importance of an asset to overall operations \\
\bottomrule
\end{tabular}
\label{tab:KPIs}
\end{table}

IoT sensors play a critical role in estimating asset KPIs and key metrics. 
%They are the primary sources of data needed to inform these KPIs and metrics. 
For instance, vibration sensors play a pivotal role in assessing a machine's Health Score, whereas temperature sensors are crucial for maintaining performance efficiency. Similarly, energy consumption meters are instrumental in calculating metrics like efficiency and Greenhouse Gas Equivalent Emissions. 
Given the diverse nature of industrial assets, including rotary equipment and fixed assets, the types of sensors required for their monitoring differ significantly. It is in this context that Large Language Models (LLMs) become valuable.
%, aiding in the generation of initial candidate sets tailored to the specific characteristics and monitoring needs of these assets.


%KPIs (Key Performance Indicators): These are strategic measures closely linked to overarching business goals. Typically fewer in number, they focus on broad business performance and the overall health of assets. KPIs are crucial for high-level decision-making and are often monitored by senior management. Examples include Overall Equipment Effectiveness (OEE) and Mean Time to Repair (MTTR).

%Metrics: These represent a broader range of operational measurements detailing various aspects of asset performance. More numerous than KPIs, metrics provide granular insights for daily management and are predominantly used for functional enhancements monitored by the operational staff. Examples include metrics like uptime, downtime, response time, and the maintenance task completion rate.



\begin{comment}
\begin{figure}[h]
\includegraphics[width=8cm]{images/common_problems.png}
\caption{Data-Driven Oriented Industrial Solutions}\label{fig:industrical_solution}
\end{figure}
\end{comment}

\begin{comment}
\begin{table*}[htbp]
\centering
\caption{Illustrated KPIs in Industrial Asset Management}
%\vspace{3mm} % Adds space 
\begin{tabular}{|c|p{6cm}|p{6cm}|}
\hline
\textbf{KPI} & \centering \textbf{Usage} & \centering \textbf{Relation to Sensor Data} \tabularnewline
\hline
Asset Reliability & Measures the frequency of asset functioning without failure. & Based on data from operational sensors, like run-time counters and performance monitors. \\
\hline
Maintenance Costs & Tracks the costs associated with maintaining an asset. & Sensor data on wear and tear can predict maintenance needs, optimizing costs. \\
\hline
Asset Availability & Proportion of time an asset is operational and available for use. & Sensors track the operational status and downtime of the asset. \\
\hline
Performance Efficiency & Assesses the operational effectiveness of an asset. & Utilizes data from sensors monitoring output levels, energy consumption, etc. \\
\hline
%Failure Probability & Predicts the likelihood of asset failure. & Based on various sensor inputs indicating deteriorating conditions or anomalies. \\
%\hline
Health Score & Reflects the current condition and performance of an asset. & Integrates data from condition monitoring sensors like vibration and temperature. \\
\hline
Sustainability Score & Evaluates the environmental sustainability of asset operations. & Informed by sensors tracking emissions, energy usage, and waste production. \\
\hline
Reliability Score & Indicates the dependability of an asset over time. & Derived from historical data and real-time monitoring via various sensors. \\
\hline
Criticality Score & Assesses the importance of an asset to overall operations. & Based on data analysis of the asset's impact on operations and production. \\
\hline
\end{tabular}\label{tab:KPIs}
\end{table*}
\end{comment}


\begin{comment}
\begin{table*}[ht]
\centering
\begin{threeparttable}
\caption{Two of the Ten Industrial Asset Classes and Their Explanations}
\vspace{0.5mm} % Adds space between the title and the table
\label{tab:asset_class_explanation}
\begin{tabular}{|>{\raggedright}p{3cm}|>{\raggedright\arraybackslash}p{15cm}|}
\hline
\multicolumn{1}{|c|}{\textbf{Asset Class}} & \multicolumn{1}{c|}{\textbf{Asset Explanation(*)}} \\ \hline
Wind Turbine & A wind turbine is a tall tower with long, spinning blades that capture the wind's energy. The wind pushes the blades around, which turns a shaft that connects to a generator. The generator converts the mechanical energy of the spinning shaft into electricity that we can use in our homes and businesses. \\ \hline
Substation Electrical Transformer & A substation electrical transformer is a large electrical device that changes the voltage of electricity. It's like a gear on a bike, but instead of changing the speed of the pedals, it changes the power of the electricity. High-voltage electricity from power plants travels through transmission lines to substations. The transformer steps down the voltage to a safer level for distribution lines, which send the electricity to homes and businesses. \\ \hline
\end{tabular}\label{tab:asset_classes}
\begin{tablenotes}
\item[*] Although both \textit{Asset Class} and \textit{Asset Explanation} are utilized in the prompts (Appendix~\ref{sec:promt_design}). The only TRUE required input is the \textbf{Asset Class} as the \textit{Asset Explanation} itself is also generated through LLM.
\end{tablenotes}
\end{threeparttable}
\label{table:note}
\end{table*}    
\end{comment}

\begin{figure}[h]
\vspace{-0.1in}
\includegraphics[width=7cm]
{images/wind_turbine_taxonomy.drawio.png}
\vspace{-0.1in}
\caption{KPI-centric Taxonomy for Asset Health Score}\label{fig:kpitree}
\end{figure}

\subsection{KPI-centric Taxonomy}\label{subsec:KPI-centric_taxonomy}
A KPI-centric taxonomy is a tree-like structure that encapsulates the domain knowledge of a specific KPI and key metric. The root node of the taxonomy tree is the KPI/metirc, while the child nodes are factors that influence the KPI/metric. The leaf nodes are either factors or sensors, annotated by asset types. The edges represent the relationships between the parent and child nodes.

For instance, Figure \ref{fig:kpitree} shows a taxonomy for the asset health KPI, where the health of an asset is analyzed by component quality, etc. By traversing the taxonomy from top to bottom, the domain knowledge of asset health for an industrial asset can be obtained. It's important to note that the taxonomy doesn't include asset-specific information, as LLM helps generate this knowledge.

Although we assume that the KPI-centric taxonomy is available as input, it's not necessary to assume that it has captured all the information. Overall, taxonomy allows domain experts to contribute their specialized knowledge, which is vital for contextualizing the solution within its specific industrial setting.

% However a generic LLM cannot understand a tree structure by default, we translate the taxonomy into text by the following format: <special formatting here TBD> [parent] is [relation] by [child] Thus, the textual interpretation of Figure 3 is: <special formatting here TBD>
%asset health is analyzed by component quality
%asset health is analyzed by historical record
%asset health is analyzed by asset profile
%component quality is impacted by mechanical health
%component quality is impacted by electrical health
%component quality is impacted by thermal health
%component quality is impacted by chemical health
%mechanical health is measured by on-demand inspection ...


\subsection{Solution Recipe}
To support the function of predicting/estimating a KPI for an industrial asset, we generate a solution entity named \textit{recipe}. For an industrial asset class, a \textit{recipe} is a collection of documentation and programming codes denoted by \(R = \{a_1, a_2, \ldots, a_n\}\). Each recipe $R$ is designed to handle a specific KPI or key metric. Currently, we break down a recipe into five artifacts, including:

\begin{itemize}
    \item \textbf{Knowledge Document for KPI/metric Analysis}: is a markdown file that provides a comprehensive introduction to the asset, including its definition and a detailed overview of the factors and sensors or another measurement such as inspection, sampling, and historical record and asset profile that could affect the KPI/metric estimation or forecasting.  
    \item \textbf{KPI/metric Modeling Configuration(s)}: one or more YAML file(s) that specifies the detailed information regarding each sensor and historical records, including description, unit if required, and value range when the value is in a normal or abnormal state or situation, etc. and the assignment of the scale to the value.
    \item \textbf{Sample Dataset}: Typically, it is a CSV (comma-separated value) dataset including identified sensor time series, variables from historical records, or asset profiles. They can be real-world industry data or synthetic data generated based on a simulated program (itself could be parts of the recipe). 
    \item \textbf{Modeling Code}: programming classes or functions that predict or estimate a KPI/metric from sensors' or other monitored data and historical or profile information. These models can be either data-driven or traditional engineering models.
    \item \textbf{Recipe Wrapper}: is an artifact that encapsulates the code for integrating inputs from both configuration settings and the dataset, and subsequently invoking the model code to facilitate model generation. 
    % By leveraging MLOps, the Recipe Wrapper facilitates comprehensive tracking of model versions and performance metrics, ensuring an organized repository of model iterations.
\end{itemize}

Large Language Models (LLM), such as ChatGPT, LLama, Mixtral, and Granite, are trained on vast multi-domain textual data curated from various sources, including books, literature, and texts gathered from online resources. These models, with their multifaceted knowledge, are not only capable of providing domain-specific insights but also generating programming code based on user instructions. In this paper, we present a solution that leverages LLM and KPI-centric taxonomy to automatically generate a \textit{recipe}.

%In the industrial domain, the collaboration is essential among various roles, such as subject matter experts (SMEs), data scientists, and software engineers. Communication between different roles are the crucial factor for the team productivity and asset management success. Since 


% In system prompt engineering, we can define three roles in the area of industrial asset management. 
% 1. SME (TBD)
% 2. Data Scientist (TBD)
% 3. Software Engineer (TBD)

% \textcolor{red}{Shuxin, combine this with the roles you are going to define - Joe.  Firstly, business decision-makers play a pivotal role in defining the Key Performance Indicators (KPIs) and key metrics which are central for the monitoring and decision support. Following this, domain experts contribute their specialized knowledge, which is vital for contextualizing the solution within its specific industrial setting. Concurrently, data scientists acquire and prepare relevant data, and further advance the development by constructing and refining predictive models. Additionally, system architects are tasked with integrating these models and other artifacts into a cohesive model deployment framework.}

% By doing proper prompting for each roles, LLMs can help creating a  \textit{Recipe} for a specific industrial asset with minimum human efforts. This hugely increases the productivity and bridges the communication gap between these diverse personas, facilitating more effective problem-solving and decision-making processes.

%\subsection{Requirement of Verfication} 

% i will move it to some where else...
%A key factor for success in applying LLMs is the assumption that the LLMs can instantly generate the necessary artifacts with accepatble quality. However, this raises a critical question: how can we trust the outcomes produced by LLMs, given their propensity for generating hallucinations? Ensuring the reliability of these results necessitates a robust verification process. This process must thoroughly justify the extracted knowledge, ensuring it is accurate and complete. The challenge of verifying the accuracy and completeness of information derived from LLMs is significant. Addressing this issue is essential for practically applying LLM-generated artifacts in developing dependable solution recipes.

==> sections/problem_formulation_save.tex <==
\section{Problem Formulation}
\vspace{10pt}

The proposed solution in this paper revolves around a systematic approach to harnessing the capabilities of Large Language Models (LLMs) for industrial management. This approach is designed to effectively bridge the gap between domain-specific knowledge and data science, leading to more efficient and adaptable industrial solutions for conditional asset management. 

\subsection{Motivation}
\vspace{10pt}

The motivation for this research into Condition-Based Maintenance (CBM) stems from the critical need to evolve industrial asset management practices in response to the rapid advancements in Industry 4.0 and the Internet of Things (IoT). Traditional asset management strategies, largely predicated on fixed schedules and standardized practices, are increasingly inadequate in the face of the dynamic, data-rich environments of modern industries. The emergence of interconnected sensors and sophisticated data analytics capabilities calls for a more responsive, efficient approach. CBM, driven by real-time data and predictive insights, offers a promising alternative. It not only aims to enhance operational efficiency and reduce downtime but also seeks to integrate cutting-edge technologies like Large Language Models (LLMs) and meta-taxonomies. This integration is expected to revolutionize asset management by enabling more nuanced, data-informed decision-making processes. The research is driven by the vision of seamlessly bridging the gap between granular sensor data and strategic asset management, thereby aligning industrial practices with the evolving landscape of digital transformation and smart factory initiatives.

Today, organizations are actively considering the adoption of GenAI as a means to boost productivity significantly. Initial evidence suggests a substantial increase in efficiency, potentially by a large margin (further research could provide specific percentages). The foundation of this potential lies in the fact that Large Language Models (LLM), including pre-trained models like ChatGPT, GPT, and Granite, are trained on extensive multi-domain textual data encompassing books, literature, and code. This diverse training has endowed these models with multifaceted knowledge, making them not only capable of providing domain-specific insights but also generating code—a dual capability that is truly transformative.

In the industrial domain, where collaboration is essential among various roles such as subject matter experts (SMEs), data scientists, and software engineers, the application of LLMs presents a compelling opportunity to scale productivity. One of the key benefits of leveraging LLMs is bridging the communication gap between these diverse personas, facilitating more effective problem-solving. This is particularly crucial in addressing the challenge of aging expertise in Asset Performance Management solutions, a significant gap in many organizations.

The complexity of the industrial sector, with potentially thousands of asset classes and their various components, places a heavy reliance on data scientists for building AI/ML models. This dependency often creates bottlenecks, especially when SMEs are unavailable to impart crucial domain knowledge. For instance, while data scientists might focus on the technicalities of machine learning models like Random Forest, SMEs are more inclined towards discussing KPIs and associated metrics. The integration of GenAI can effectively mitigate these challenges by providing a platform where both technical and domain-specific knowledge are seamlessly integrated, enhancing the efficiency and accuracy of AI/ML model development in industrial applications.

By embracing GenAI, we aim to not only streamline the model development process but also to ensure that the invaluable insights and expertise of SMEs are effectively captured and utilized, even in their absence. This approach promises to revolutionize the way we manage and optimize industrial assets, leading to more informed decision-making and significantly improved operational outcomes.

In addressing the business challenges associated with a specific asset type, the initial step involves identifying the pertinent business problem and quantifying it through relevant Key Performance Indicators (KPIs). The solution to this problem hinges on the creation of a customized solution recipe. This recipe is designed to seamlessly integrate with the existing IoT infrastructure deployed for the asset. Once instantiated, the recipe should provide a tailored solution catering to the unique needs of a specific client.

The realization of this solution encompasses a series of components, collectively forming a comprehensive set of prompts:

    Output Components:
        Documentation: Detailed guides and references outlining the solution’s framework and operational parameters.
        Configuration File: Essential for setting up and customizing the solution to align with specific client requirements and asset characteristics.
        Sample Dataset: A representative data set that facilitates the understanding and calibration of the solution within the given context.

    Code for Modeling:
        The essence of the solution recipe lies in its coding, which articulates how to utilize the data effectively for modeling purposes. This code forms the backbone of the solution, translating raw IoT data into actionable insights driven by the identified KPIs.

By focusing on these components, the proposed solution recipe aims to bridge the gap between theoretical KPI modeling and practical application in the field. It ensures that once the solution is deployed, it aligns perfectly with the client's specific asset management needs, leveraging the power of IoT and advanced data analytics to address the identified business problem effectively.



\subsection{KPIs for Conditional Asset Management}
\vspace{10pt}

In Conditional Asset Management, both Key Performance Indicators (KPIs) and metrics are essential tools used to assess and improve the performance, reliability, and sustainability of assets. KPIs like Asset Reliability, Maintenance Costs, and Asset Availability provide quantifiable measures of an asset's performance and operational efficiency. Metrics such as Failure Probability, Health Score, and Greenhouse Gas Equivalent Emissions offer predictive insights and assess the risk and environmental impact of assets. These measures are crucial for making informed decisions about maintenance, resource allocation, and long-term asset strategies.

Sensors play a vital role in gathering the necessary data for these KPIs and metrics. For instance, vibration sensors can inform the Health Score of a machine, while temperature sensors are crucial in monitoring and maintaining optimal performance efficiency. Energy consumption meters are key in calculating Greenhouse Gas Equivalent Emissions. The integration of sensor technology with asset management systems enables real-time monitoring and analysis, providing a comprehensive view of asset health and performance.

\begin{table*}[htbp]
\centering
\begin{tabular}{|c|p{6cm}|p{6cm}|}
\hline
\textbf{KPI/Metric} & \centering \textbf{Usage} & \centering \textbf{Relation to Sensor Data} \tabularnewline
\hline
Asset Reliability & Measures the frequency of asset functioning without failure. & Based on data from operational sensors, like run-time counters and performance monitors. \\
\hline
Maintenance Costs & Tracks the costs associated with maintaining an asset. & Sensor data on wear and tear can predict maintenance needs, optimizing costs. \\
\hline
Asset Availability & Proportion of time an asset is operational and available for use. & Sensors track operational status and downtime of the asset. \\
\hline
Performance Efficiency & Assesses the operational effectiveness of an asset. & Utilizes data from sensors monitoring output levels, energy consumption, etc. \\
\hline
Failure Probability & Predicts the likelihood of asset failure. & Based on various sensor inputs indicating deteriorating conditions or anomalies. \\
\hline
Health Score & Reflects the current condition and performance of an asset. & Integrates data from condition monitoring sensors like vibration and temperature. \\
\hline
Sustainability Score & Evaluates the environmental sustainability of asset operations. & Informed by sensors tracking emissions, energy usage, and waste production. \\
\hline
Reliability Score & Indicates the dependability of an asset over time. & Derived from historical data and real-time monitoring via various sensors. \\
\hline
Criticality Score & Assesses the importance of an asset to overall operations. & Based on data analysis of the asset's impact on operations and production. \\
\hline
\end{tabular}
\caption{KPIs and Metrics in Conditional Asset Management}
\end{table*}

\subsection{Meta-Taxonomy for Asset Management}
\vspace{10pt}

\begin{figure}[h]
\includegraphics[width=8cm]{images/concept_flow.png}
\end{figure}

We are engaged in tasks that involve knowledge and reasoning, focusing on the AI Mental Model, which encapsulates the cognitive module within the AI system. This model is instrumental in delineating the process of parsing and comprehending information or interactions to construct effective solutions, particularly for specific industrial assets. To facilitate this, we utilize a flowchart that guides our approach in interpreting data and making informed decisions. This approach is crucial in understanding how the AI system processes information and arrives at solutions tailored to the unique demands of our industry.

The following figure displays the problems with conditional asset maintenance. 

\begin{figure}[h]
\includegraphics[width=8cm]{images/common_problems.png}
\end{figure}

We need to standardize the Problems faced by conditional asset management.  We start with categorizing business problems into different groups based on their nature and focus areas in asset management. Here's a summary of these problems grouped into relevant categories:

\subsection{KPI-Oriented Operation}
\vspace{10pt}

KPI allows up to directly match the results with the decision support.  

KPI-oriented monitoring is crucial for Conditional Asset Management for several compelling reasons. This approach aligns the monitoring process with key performance indicators (KPIs) that are critical to the organization's objectives and asset performance. Here's why it's essential:

Focused Performance Tracking

    Targeted Monitoring: KPI-oriented monitoring ensures that the focus is on metrics that directly impact asset performance and organizational goals.
    Prioritization: Helps in prioritizing monitoring efforts on aspects that are most critical to asset health and operational efficiency.

2. Data-Driven Decision Making

    Informed Decisions: By monitoring KPIs, decisions regarding maintenance, repairs, and replacements are based on quantifiable data rather than assumptions or estimations.
    Objective Assessment: KPIs provide an objective basis for assessing the condition and performance of assets.

3. Enhanced Predictive Maintenance

    Proactive Approach: KPIs can indicate emerging issues before they become critical, allowing for proactive maintenance and interventions.
    Reduction in Downtime: Timely maintenance based on KPI trends can significantly reduce unplanned downtime.

4. Cost Optimization

    Resource Allocation: KPIs help in identifying areas where resources should be allocated for maximum impact, optimizing maintenance and operational costs.
    Lifecycle Cost Management: Monitoring KPIs like asset lifecycle costs aids in making informed decisions about repairs, replacements, and investments.

5. Improved Asset Reliability and Longevity

    Asset Health: Continuous monitoring of KPIs related to asset health ensures that assets are maintained in optimal condition.
    Extended Asset Life: By addressing issues early and maintaining assets effectively, their operational lifespan can be extended.

6. Regulatory Compliance and Safety

    Compliance Monitoring: Certain KPIs can be crucial for ensuring compliance with industry regulations and standards.
    Safety Assurance: Regular monitoring of safety-related KPIs helps in maintaining a safe working environment.

7. Strategic Planning and Reporting

    Strategic Insights: KPI trends provide insights for strategic planning and future investments in assets.
    Performance Reporting: KPIs offer a clear and measurable way to report on asset management performance to stakeholders.

8. Adaptability and Continuous Improvement

    Responsive to Changes: KPI-oriented monitoring allows for quick adaptation to changes in asset performance or operational conditions.
    Basis for Improvement: Continuous analysis of KPIs provides a basis for ongoing improvement in asset management practices.

In summary, KPI-oriented monitoring in Conditional Asset Management ensures that monitoring efforts are aligned with the most critical aspects of asset performance and organizational objectives. It enables a more strategic, efficient, and effective approach to managing assets throughout their lifecycle.



\subsection{Standardization of Model Approaches}
\vspace{10pt}


\subsubsection{Engineering Problems}
\vspace{10pt}

\textbf{Energy Loss and Efficiency}

Energy efficiency and loss in electrical transformers are critical KPIs directly influencing power systems' overall performance and cost-effectiveness.  They are also important indicators of the electrical transformer's health and the making of the decision for the replacement.  There are non-load loss and load loss for electrical transformers.   This document provides the empirical approaches to estimate the load loss, the significant portion of energy loss.


\textbf{Environment Emissions - CO2e}

The calculate the CO2 equivalent emissions from the amount of energy usage or lost due to inefficiency, starting with the example of energy loss from an electrical distribution transformer. The method can be used for all kinds of equipment to determine how much CO2 equivalent emissions they effectively put into the environment.

In one example, we first calculate the energy loss and then, based on the location of the electrical transformer specified with the US location ZIP code, calculate the emissions. Inside the calculation, we use the information published by the USA EPA. 

\textbf{Rule-based anomaly}

The rule-based anomaly detection uses sensors or other deduced metrics (such as KPIs) with set maximum and minimum threshold points. This method offers a straightforward and effective means of monitoring sensor metrics or KPIs (Key Performance Indicators) over a designated period. It identifies anomalies by comparing observed values against predefined thresholds. If observed values surpass these thresholds, the system generates a tag (or indicator) for that timestamp. Additional rules tally these indicators over a specified timeframe for various metrics or KPIs to initiate an alert or anomaly. These supplementary rules help prevent an overload of anomalies in the system.

This rule-based anomaly detection method is easy to implement and understand, making it a favored choice for monitoring system performance and early detection of potential issues. However, it does have its limitations since it depends on predefined thresholds. It might not recognize more intricate or subtle anomalies that necessitate advanced statistical or machine-learning techniques.

\subsubsection{ML Problems}
\vspace{10pt}


\subsection{Selection of the Appropriate LLM Model}
\vspace{10pt}
Once the domain knowledge requirements are clearly defined, the next step is to select the most suitable LLM model for the task. This selection is based on several criteria, including the model's ability to understand and process domain-specific language, its performance in similar contexts, and its adaptability to the unique challenges of the industry.
Recommended Model

For this study, we recommend the Llama 2 model.  Llama 2 is a language processing technology similar to GPT 3.5 and OpenAI’s  PaLM 2.  It employs a neural network with billions of variables, using the same transformer architecture and development concepts as its counterparts. Llama 2 is one of the few open-source language models that can generate human-like responses, much like GPT-3. However, it stands out because it is fully open-source, which means all individuals have complete access to the model for any purpose. Llama 2 has demonstrated exceptional proficiency in understanding and processing complex industrial data. This model stands out due to its advanced capabilities in handling domain-specific queries and generating insightful and actionable responses.

The Llama-2-70B-chat model is a 70 billion parameter generative text model from Meta AI. It is a fine-tuned version of the Llama-2 model, which is a collection of pretrained and fine-tuned generative text models ranging in scale from 7 billion to 70 billion parameters. The Llama-2-70B-chat model is optimized for dialogue use cases and has been shown to be more effective than other models at generating natural and engaging conversations. It has also been shown to be more accurate and efficient than other models, making it a good choice for large-scale chatbot applications.

Here are some key details about the Llama-2-70B-chat model:

    Model size: 70 billion parameters
    Architecture: Transformers
    Training data: Common Crawl dataset
    Fine-tuning data: Dialogues from Reddit and other chat platforms
    Performance: More effective than other models at generating natural and engaging conversations; more accurate and efficient than other models
    Applications: Large-scale chatbots, virtual assistants, customer service bots

The Llama-2-70B-chat model is still under development, but it has already shown significant promise for a variety of applications. It is likely to become even more powerful and versatile in the future, making it a valuable tool for developers and researchers alike.


\subsection{Standardizing Domain Knowledge Acquisition through LLM}
\vspace{10pt}

The first step involves establishing a standardized process for querying the LLM to extract relevant domain knowledge. This process is crucial as it ensures that the LLM comprehensively understands and interprets the specific requirements and nuances of the industrial domain in question. The standardized query process is designed to be intuitive yet thorough, enabling the LLM to provide detailed and relevant domain insights that are crucial for the subsequent steps.

\subsection{Converting Meta-Taxonomy into Auto-Recipe}
\vspace{10pt}

The final step involves translating the domain knowledge acquired from the LLM into actionable insights within the framework of creation the industrial solution, referred to as AutoRecipe.

The AutoRecipe is a conceptual framework designed to streamline the process of model development and deployment in industrial settings. It acts as a conduit between the raw domain knowledge provided by the LLM and the practical applications within the industry. The AutoRecipe is engineered to be flexible, scalable, and adaptable, accommodating the dynamic nature of industrial management.
Introducing Recipe Automation

Within the AutoRecipe, we introduce the concept of Recipe Automation. This involves the creation of automated workflows or 'recipes' that can be applied to various industrial processes. These recipes are generated based on the domain knowledge extracted from the LLM, tailored to meet the specific needs of each industrial scenario. Recipe Automation stands at the core of AutoRecipe, embodying the principles of efficiency, accuracy, and adaptability in industrial management.


In conclusion, this Asset AI Life-Cycle flow provides a comprehensive framework for implementing condition-based maintenance using AI and a meta-model approach. It emphasizes the importance of continuous monitoring, predictive analysis, and feedback mechanisms to ensure effective maintenance strategies and asset health management.

==> sections/save_experiment.tex <==
\section{Experiment and Case Study}
\vspace{10pt}

In the dynamic field of industrial asset management, the adoption of transfer learning, augmented by the innovative use of Large Language Models (LLM), marks a significant stride toward enhanced efficiency and innovation. This section delves into the sophisticated transfer of proven models from electrical transformers to wind turbine gearboxes, a process now further refined by integrating a guided auto-recipe system. This system represents a groundbreaking approach in leveraging existing models that cover key aspects such as efficiency, CO2 emissions, health monitoring, and anomaly detection and applying them to the distinct context of wind turbine gearboxes.

We experience ten industrial assets.

\begin{figure}[h]
\includegraphics[width=8cm]{images/common_problems.png}
\caption{Industrial Solutions Overview}
\end{figure}

\begin{figure}[h]
\includegraphics[width=8cm]{images/execution_flow.png}
\end{figure}

\subsection{Experiment}
\vspace{10pt}

One of the KPIs is the health score, here is an example from IBM Maximo Asset Score~\footnote{\url{http://maximo-lab.monitordemo4.ibmmam.com/apm_8.9/asset_scores}}

The website discusses "Asset Custom Scores" in Maximo Health and Maximo Health and Predict - Utilities (HPU) within the Maximo Application Suite (MAS). It focuses on new features allowing users to create custom scores for asset conditions using either a formula-based approach or notebook-based methods deployed through Watson Studio or IBM Machine Learning Service. These custom scores help make informed repair or replacement decisions and select assets for investment projects. The page also highlights a lab exercise demonstrating how to set up and use these scores, prerequisites for the lab, and the use of Maximo Health for asset condition analysis and investment strategy optimization. The content is aimed at reliability engineers and subject matter experts in asset management.

\subsubsection{Knowledge Extraction}
\vspace{10pt}

In the experimental phase of our knowledge extraction, we meticulously tested four distinct approaches to generate outputs for the knowledge base, specifically tailored to the domain of a given Key Performance Indicator (KPI). Our initial step involved compiling a comprehensive list of questions. Among these, we identified a crucial element: the final question in our guided pipeline, which plays a pivotal role in the process.

The approaches tested are as follows:

    \begin{itemize}
        \item Single Question (SQ): This approach focuses on the last question in the guided pipeline, isolating its potential to elicit comprehensive information.
        
        \item All Questions Concatenated (AllQ): Here, we combined all questions into one extended query, testing the effect of presenting the full context in a single prompt.
         
        \item All Questions with Chain of Thought (AllQCOT): This method enhances the AllQ approach by incorporating a 'think step-by-step' comment in the prompt, guiding the LLM to process the information in a structured, sequential manner to follow a reasoning process by explicitly laying out the intermediate steps leading to the desired outcome. This approach goes beyond simply providing input and output but allows the model to "show its work" and demonstrate its understanding of the problem.
        
        \item Guided Iterative Process (GIP): This approach simulates a dynamic Q/A session, where each question and its subsequent answer lead to the next query, mirroring a real-world interaction pattern.  In this process, there are multiple Q/A generated and such answers help to understand how the final knowledge is generated for better validation with a human-in-the-loop. 
        \item 
    \end{itemize}
    
Each of these methods aims to optimize the extraction of domain-specific knowledge for a particular KPI, evaluating their effectiveness in contributing to a rich, accurate knowledge base. This experimentation is crucial in determining the most efficient approach to harnessing the capabilities of LLMs for detailed and relevant knowledge generation in industrial asset management.
        

\begin{table*}[h]
\centering
\caption{Summary of Methods and Their Advantages and Disadvantages}
\label{tab:methods_summary}
\begin{tabular}{>{\raggedright\arraybackslash}p{3.5cm} >{\raggedright\arraybackslash}p{5.0cm} >{\raggedright\arraybackslash}p{5.5cm}}
\toprule
\textbf{Method} & \textbf{Advantages} & \textbf{Disadvantages} \\
\midrule
Single Question (SQ) & Focus and precision, Simplicity in execution & May miss broader context, Limited in scope \\
\addlinespace
All Questions Concatenated (AllQ) & Contextual richness, Holistic understanding & Potentially overwhelming for the model, May produce less focused responses \\
\addlinespace
All Questions with Chain of Thought (AllQCOT) & Structured thinking, Enhanced clarity & More complex to construct, May lead to verbose responses \\
\addlinespace
Guided Iterative Process (GIP) & Dynamic interaction, Incremental learning, Customizability & Time-consuming, Requires careful question crafting \\
\bottomrule
\end{tabular}
\end{table*}


\section{Knowledge to Code}
\vspace{10pt}

\subsubsection{Sample Data Generation}
\vspace{10pt}

We have two approaches to generate the sample data.  One is directly from the code, 

\subsubsection{Experiment Categories and Objectives}
\vspace{10pt}

\subsection{How to validate?}
\vspace{10pt}

As illustrated in FigureFigure~\ref{fig:Pipelines for Artifact Generation}, the initial artifacts comprise a knowledge document outlining methods for estimating or modeling a Key Performance Indicator (KPI). Subsequent recipe artifacts are then deduced from this foundational knowledge. However, a critical aspect of our research involves validating these artifacts to ensure their utility and reliability.  It is imperative to validate knowledge document validation.

Validation hinges on two key factors: completeness and accuracy. While our current research predominantly focuses on reducing hallucinations in the generated content, our standards go beyond this. It is imperative that the generated document not only adheres to a specific format but also encompasses accurate, relevant, and comprehensive information.

Yet, assessing completeness presents a significant challenge, as it is inherently difficult to quantify. A conventional approach would involve creating a similar document manually and performing a similarity comparison. However, in our case, such pre-existing documents do not exist; this creates a 'chicken and egg' problem. Without prior knowledge or a benchmark document, evaluating the completeness of our generated artifacts becomes a complex task that may require innovative validation methodologies tailored to the unique nature of our project.


\begin{table*}[h]
\centering
\begin{tabular}{|c|l|p{10cm}|}
\hline
\textbf{No.} & \textbf{Nature of the Problem} & \textbf{Objective Description} \\
\hline
1 & Asset Efficiency & Assessing and optimizing asset efficiency. \\
\hline
2 & Greenhouse (CO2e) Contribution & Evaluating environmental impact. \\
\hline
3 & Health Assessment & Determining operational health of assets. \\
\hline
4 & Criticality Assessment & Identifying and ranking asset criticality. \\
\hline
5 & Rule-Based Anomaly Detection & Detecting mechanical, thermal, or electrical anomalies. \\
\hline
6 & Group Sensor Anomaly Detection & Identifying anomalies based on sensor data. \\
\hline
7 & Asset Maintenance/Replacement & Assessing maintenance or replacement needs. \\
\hline
\end{tabular}
\caption{Experiment Categories and Objectives}
\label{table:experiment-categories}
\end{table*}



\subsubsection{Experiment Components}
\vspace{10pt}

Each problem category involves three key components: 
\begin{itemize}
    \item \textbf{Documentation:} Structure and format of Markdown files for documentation.
    \item \textbf{Configuration:} Model configurations and parameter adjustments.
    \item \textbf{Python Code:} Python code structure, compatibility with MLFlow and Model Factory.
\end{itemize}


\subsection{Case Study - Health Score for Industrial Assets}
\vspace{10pt}


Using the health score as an example,  we separate the health score analyzed from three aspects:
1. the component qualities; 
2. the historical records;
3. the asset ages.

We develop the health score for each of the aspects independently.  The end-user has the freedom to select and choice which aspects based on the data availability. 


\subsubsection{Rule-based Anomaly Transfer Learning}
\vspace{10pt}

Here should the configuration files are posted. 

\subsubsection{Model-Drive Anomaly Transfer Learning}
\vspace{10pt}


\subsubsection{Health Score Transfer Learning}
\vspace{10pt}


\subsubsection{Performance Efficiency Transfer Learning}
\vspace{10pt}



\subsection{Validation}
\vspace{10pt}

There are multiple validations required for the recipe for the artifacts.  Certain artifacts are likely to be validates. 

==> sections/solution_outline_save.tex <==
\section{Solution Outline}
\vspace{10pt}

\textcolor{red}{Make a discussion of standardizing and specification - standardizing for the prompting generation for a given KPI and specification to involve the asset information}
As we delve into the solution phase of our research, understanding the role of Large Language Models (LLMs) in our methodology is crucial. Our work harnesses LLMs for logical reasoning and problem-solving, specifically in developing models to calculate Key Performance Indicators (KPIs) or key metrics real-time sensor data and historical records as inputs. This specialized form of logical reasoning is directed towards modeling development for distinct industrial challenges, moving beyond general problem-solving as current LLM research focused on.

Our task diverges from simplistic endeavors like Sudoku; it demands nuanced, guided reasoning and precise prompt practices. This constrained reasoning approach is essential due to the inherent limitations in current LLMs for complex reasoning tasks. Our proposed solution involves developing a system for the calculation or estimation of KPIs and metrics, specifically tailored to individual industrial assets. This approach showcases the efficacy of LLMs in a structured reasoning framework, differentiating our problem-solving horizon.  In addressing specific asset-related business challenges, our initial step is to identify and quantify the business problem through relevant KPIs. The core of our solution is the creation of a custom solution recipe, designed to integrate seamlessly with the existing solution framework and cater to unique client needs for specific KPIs requirement, IoT framework, and management data availability.

Furthermore, our focus extends to tasks involving knowledge extraction and reasoning, particularly centered around the AI Mental Model (meta-taxonomy. This model plays a pivotal role in parsing and understanding information to construct practical solutions for industrial assets. We employ a flowchart to guide our data interpretation and decision-making processes, which is critical for the AI system to provide solutions that meet the unique demands of our industry.

Ultimately, we anticipate generating a set of artifacts that can be directly applied or modified to suit different client requirements. This outcome is a testament to the adaptability and precision of our approach, setting a new benchmark in the field of industrial asset management.

\subsection{Architecture}
\vspace{10pt}

\begin{figure}[h]
\includegraphics[width=8cm]{images/architecture.drawio.png}
\caption{Architecture Diagram for AutoRecipe Generation}
\end{figure}


In the architectural design phase of our CBM solution development, a multifaceted uapproach is adopted to incorporate the essential roles that contribute to a successful implementation. Firstly, business decision-makers play a pivotal role in defining the Key Performance Indicators (KPIs) and metrics which are central to the targeted objectives. Following this, domain experts contribute their specialized knowledge, which is vital for contextualizing the solution within its specific industrial setting. Concurrently, data scientists acquire and prepare relevant data, and further advance the development by constructing and refining predictive models. Additionally, system architects are tasked with integrating these models and other artifacts into a cohesive model deployment framework.

Central to this architecture is the development of a versatile large language model (LLM) pipeline. The LLM's role is strategically evolved to respond effectively to queries generated from the meta-taxonomy, facilitating a dynamic and intelligent interaction between the system and its data inputs. This sophisticated interplay between the LLM and the meta-taxonomy is crucial for extracting actionable insights, which are then seamlessly incorporated into the CBM framework, ensuring a data-driven and contextually relevant solution.

This architecture optimizes workflow and enhances output quality, ensuring a seamless integration with the LLM.  Our system's architecture is designed to streamline the thought process and output generation, leveraging a sophisticated meta-taxonomy as its core component. This meta-taxonomy records and categorizes the thought process, ensuring a structured and comprehensive approach. Central to the system is the 'Prompt Register,' a dynamic repository (Prompt Registry) that stores and manages the prompts used to interact with the system. 

Between the meta-taxnomy and the prompt registry is a parser and question generator.  We stored the meta-taxonomy as a graph represented using YAML; we invoked a parser to extract the logic flow, entity, and relationship from the graph representation.  Then, we feed this into another tool developed named \textbf{AutoQ} to generate the questions for us.  The details of the \textbf{AutoQ} are beyond this paper and will be discussed in another paper.  

Role of LLM: At the top left, there is a group of Pseudo-human roles that LLM contribute to the system, including a System Architect, Data Scientist, and Domain Expert. Each role has assigned a dedicated system prompt to define its role. These roles are responsible for providing expertise, generating configuration file and developing models to the system.
Prompt Registry: Below the pseudo-role, there is a "Prompt Registry," which seems to be a storage system for prompts. This could be where the user-prompt inputs to the LLM are stored and managed.
Templates: Linked to the Prompt Registry, there are "Templates," which may be pre-defined structures or formats that prompts or outputs adhere to. Additionally, a specialized template module is integrated, tasked with defining the format and structure of the outputs for various artifacts. This ensures a consistent and standardized output across different applications. 
Auto-Recipe: This component receives input from the human resources and seems to automate a part of the process, possibly by selecting or generating prompts based on predefined criteria.
Workflow (Meta-taxonomy): The Auto-Recipe feeds into the Workflow, which could be the set of rules or logic that the system follows to process data. "Meta-taxonomy" suggests a hierarchical organization of the workflow steps or categories.
KB Library (Artifacts): Parallel to the Workflow, there's a Knowledge Base Library that stores artifacts. These artifacts might be outputs, references, or data models that the system uses or produces.
LLM: On the far right, there is an LLM, which stands for Large Language Model. This is likely the core processing unit where the AI does its computational work, such as language understanding, generation, and prediction.
Deployment Platform: All of these components are situated over what is labeled as the Deployment Platform, indicating the underlying infrastructure that supports the deployment and operation of the system.
Overall, the flowchart describes a system where human experts design and provide data to a system that uses templates and a prompt registry to automatically generate workflows and utilize a knowledge base, all orchestrated through a Large Language Model and deployed on a platform.



The proposed solution recipe aims to bridge the gap between theoretical KPI modeling and practical application by focusing on these components. It ensures that once the solution is deployed, it aligns perfectly with the client's specific asset management needs, leveraging the power of IoT and advanced data analytics to address the identified business problem effectively.

Our system's architecture leverages a sophisticated meta-taxonomy, denoted as \(T\), to record and categorize the thought process. This taxonomy \(T\) is a structured set, where each element \(t_i \in T\) represents a unique category or aspect of the tho. The 'Prompt Register', represented by \(P\), is a dynamic repository where each prompt \(p_j \in P\) is stored and managed. The output format for various artifacts is defined by a template function \(F(x)\), where \(x\) represents the input parameters and \(F\) dictates the structure of the output. Our 'Knowledge Base', symbolized by \(K\), is a storage for all generated artifacts, where each artifact \(a_k \in K\) is readily accessible for future use.

The communication pipeline with the Large Language Model (LLM) is modeled as a function \(L(P, K) \rightarrow A\), where \(P\) and \(K\) are inputs from the Prompt Register and Knowledge Base respectively, and \(A\) represents the artifacts output. Additionally, a 'Recipe' is defined as a collection of artifacts, denoted by \(R = \{a_1, a_2, \ldots, a_n\}\), where each recipe \(R\) is designed to handle a specific KPI and metric. This collection of artifacts \(R\) can be utilized as the base for deployment.

\subsection{Pipelines for Artifact Generation}
\vspace{10pt}




\begin{figure}[h]
\includegraphics[width=8cm]{images/artifact_generation_pipeline.drawio.png}
\caption{Chained Pipelines for Decomposing Higher Level task into Smaller and Actionable Prompt Technique for Artifact Generation}\label{fig:Pipelines for Artifact Generation}
\end{figure}


From Figure~\ref{fig:Pipelines for Artifact Generation}, we have three pipelines to generate artifacts for a recipe.  For a selected pipeline, each stage is a step in a continuous process, leading from domain knowledge generation to a deployable solution for real-time monitoring and predictive maintenance for an asset, such as a wind turbine. The domain expert's insights about the asset initiates the pipeline, guiding the data scientist in creating a tailored model. The pipeline structure emphasizes the streamlined, sequential flow from one stage to the next, embodying a systematic approach to developing a health monitoring system for the wind turbine.

Domain Expert Pipeline

    Initialization: A domain expert triggers the pipeline with a detailed query about a wind turbine's component health monitoring.

    Configuration Creation: The expert compiles a configuration file detailing the sensors responsible for monitoring the health of various wind turbine components.

    Health Status Labeling: The configuration file includes criteria for labeling the output of each sensor to indicate the health status of the monitored component (e.g., normal, warning, critical).

Data Scientist Pipeline (Input Preparation)

    Input Configuration: The data scientist, following the pipeline's sequence, uses the domain expert’s configuration file to define model input parameters.

    Simulated Dataset Assembly: The scientist prepares a simulated dataset containing sensor output data, annotated with health status labels to reflect different operational states of the wind turbine.

    Knowledge Base Storage: The configuration settings and the simulated dataset are stored in a knowledge base, serving as a repository for the pipeline's artifacts.

Data Scientist Pipeline (Model/Code Construction)

    Model Generation: The pipeline advances to auto-generate modeling code capable of interpreting sensor data in the context of component health.

    Code Testing: Alongside the modeling code, testing scripts are generated to validate the model's accuracy against the simulated dataset.

    Data Formatting: The pipeline ensures the sensor data is formatted correctly for model consumption, restructuring it as necessary.

    Operational Wrapper Creation: A wrapper encapsulates the modeling and testing environment, allowing for the deployment and operation of the model with actual sensor data from the wind turbine.


\begin{itemize}
    \item \textbf{Artifact Name:} Lists the various artifacts like Markdown Document, Configuration, etc., each representing a distinct component of the project.

    \item \textbf{Input Requirement:} Specifies the prerequisites for each artifact, such as specific content for the Markdown Document and system specifications for Configuration.

    \item \textbf{Explanation of Output:} Describes the nature and format of each artifact's output, like the Markdown format for the Markdown Document and operational parameters for Configuration.

    \item \textbf{Prompt Engineering Practices:} Provides guidance on best practices for creating each artifact, advising on clarity for prompts, data relevance, and adherence to coding standards.

\end{itemize}

\begin{table*}[ht]
\centering
\caption{Artifacts from LLM Pipelines}
\vspace{1mm} % Adds space between the title and the table
\label{tab:artifacts}
\begin{tabular}{|>{\raggedright}p{3cm}|>{\raggedright}p{4cm}|>{\raggedright}p{4cm}|>{\raggedright\arraybackslash}p{5cm}|}
\hline
\textbf{Artifact Name} & \textbf{Input Requirement} & \textbf{Explanation of Output} & \textbf{Prompt Engineering Practices} \\ \hline
Knowledge Document & A meta-taxonomy designed for a KPI and asset class name & A document detailing the project, its goals, and methodology. & Prompt-verification to enforce the focus on the KPI and asset class, step-by-step prompts of document output \\ \hline
Configuration & Configuration parameters & Configuration files or parameters used in the project. & template and example \\ \hline
Sample Data & Data source & A sample of the data used in the project for testing or demonstration purposes. & template and example \\ \hline
Code for Data Transfer & Source and Destination Details & Code responsible for transferring data between systems or modules. & - \\ \hline
Code for Modeling & Data, parameters & The main modeling code used in the project for analysis or prediction. & - \\ \hline
Test Code for Modeling as Unit Test & Test cases, data & Code that tests the modeling components to ensure they work as expected. & - \\ \hline
Recipe Code & Instructions, guidelines & Step-by-step code for replicating a specific process or result. & - \\ \hline
\end{tabular}
\end{table*}




\subsubsection{Standardization of Modeling}
\vspace{10pt}

All models, machine learning models, or engineering formulas can be conceptualized as $f(X) = y$ functions. For consistency, it's imperative to standardize these models into a uniform format. This standardization should ensure compatibility with Scikit Learn's framework. To achieve this, let's consider creating a class that extends \textit{BaseEstimator} and \textit{TransformerMixin} from Scikit Learn. This class would handle two primary inputs: a configuration file and a data frame. The data frame will encompass multiple assets, with each row detailing the health score of a specific component. By designing this class, we can efficiently process and integrate diverse models within a Scikit Learn-compatible pipeline.


\subsection{Integration with LLM}
\vspace{10pt}

Recent advancements in large language models (LLMs) have pushed the boundaries of natural language processing, but these models often grapple with efficiency and scalability. Mixtral-8x7B offers a unique approach, introducing a modular architecture comprised of eight specialized expert networks, each trained on 7 billion parameters. This departs from the traditional monolithic LLM design, focusing on task-specific expertise and collaborative processing.

Each expert in Mixtral-8x7B tackles distinct aspects of language understanding, potentially including contextual analysis, semantic interpretation, syntactic parsing, and pragmatic inferences. At each processing layer, a dynamic router selects two experts to handle the input based on its current state. The outputs of these experts are then combined to guide the subsequent layer, leveraging the combined knowledge and skills of the team.
Unlike traditional monolithic LLMs, Mixtral-8x7B boasts eight specialized "expert" networks. These task-focused teams collaborate, tackling language challenges like analysis and interpretation. This unique design offers efficiency, achieving top performance in tasks like summarization, even compared to larger models. Further, its modularity allows customization for specific needs, making Mixtral-8x7B a versatile LLM poised for diverse applications.





